From Profiling to Optimization: Unveiling the Profile Guided Optimization

Profile Guided Optimization (PGO) uses runtime profiling to direct compiler optimization decisions, effectively combining static analysis with actual execution behavior to enhance performance. Runtime profiles, collected through instrumentation or hardware- and software-assisted sampling, provide detailed insights into control flow, branch predictions, and memory access patterns. This survey systematically categorizes PGO research by profiling method (instrumentation vs. sampling), optimizations (compile time and link/post-link time), compiler integration (GCC, LLVM), and target architectures. Key algorithms and frameworks are shown in terms of design principles. Performance evaluation on representative examples demonstrates PGO's speedups, overheads, and integration maturity. Finally, we identify open challenges, such as reducing sampling overhead, dynamic input workloads, and supporting cross-architecture portability, and propose future research directions to low-overhead profiling and advanced compilers.

==> contents/figs/gcc-vs-llvm.tex <==
\begin{figure}[htbp]
  \centering
  \scriptsize
  \begin{tabular}{lcc}
    \toprule
    \textbf{Build Phase} & \textbf{GCC 12.2} & \textbf{LLVM 15} \\
    \midrule
    Compile Time &
      \begin{tabular}[t]{@{}l@{}}
        Instrumentation PGO: `-fprofile-generate` / `-fprofile-use` \\
        AutoFDO: `-fauto-profile=<afdo>` \\
        Inlining, loop unrolling, branch reordering, value specialization
      \end{tabular} &
      \begin{tabular}[t]{@{}l@{}}
        Instrumentation PGO: `-fprofile-instr-generate` / `-fprofile-instr-use` \\
        AutoFDO: `-fprofile-sample-use` \\
        Block reordering, inlining, hot/cold splitting
      \end{tabular} \\
    Link Time &
      \begin{tabular}[t]{@{}l@{}}
        LTO merges profiles (`.gcda` / `.afdo`) \\
        Cross-module inlining and layout
      \end{tabular} &
      \begin{tabular}[t]{@{}l@{}}
        LTO merges `.profdata` and samples \\
        IR-level interprocedural optimizations
      \end{tabular} \\
    Post-Link Time &
      \begin{tabular}[t]{@{}l@{}}
        No built-in passes; optional BOLT
      \end{tabular} &
      \begin{tabular}[t]{@{}l@{}}
        External BOLT / Propeller for layout
      \end{tabular} \\
    \bottomrule
  \end{tabular}
  \caption{PGO and AutoFDO in GCC 12.2 vs LLVM 15 Across Build Phases}
  \label{fig:pgo_phase_comparison}
\end{figure}

==> contents/sections/sec4_5_compiler.tex <==
\subsection{Compiler Comparison}
% \subsection{编译器对比}

In the previous sections, we systematically reviewed the theoretical foundations of profile-guided optimizations. In this section, we examine two leading industrial compilers --- GCC 12 and LLVM 15 --- to analyze in depth how they integrate profile-guided techniques into their compilation pipelines and how these techniques interact with conventional optimizations.
% 在前文中，我们系统梳理了反馈优化技术的理论基础，本节将主要介绍主流工业级编译器——以 GCC 12.2 与 LLVM 15 为例，深入剖析它们如何在编译流程中引入反馈优化，如何与常规优化技术协同工作。
TODO:
% connect next section with the previous one

% \input{contents/tables/gcc-llvm.tex}

% GNU Compiler Collection (GCC) is an open-source compiler suite led by the Free Software Foundation (FSF). Widely adopted in both industry and academia, GCC provides a mature and stable front-end and mid/back-end optimization pipeline, along with advanced features such as loop unrolling, function inlining, auto-vectorization, and Profile-Guided Optimization (PGO). Its modular design and rich plugin interface allow flexible integration of third-party analysis tools and custom optimization passes, making GCC a key platform for compiler research and high-performance software development.
% GNU 编译器集合（GCC，GNU Compiler Collection）是由自由软件基金会（FSF）主导开发的开源编译器,作为工业界和学术界广泛采用的编译器，GCC 不仅提供成熟稳定的前端与中后端优化管线，还内置了诸如循环展开、函数内联、自动向量化以及 Profile-Guided Optimization（PGO）等高级优化功能。此外，GCC 的模块化设计和丰富插件接口使其能够灵活集成第三方分析工具与自定义优化通道，是研究编译器技术和构建高性能软件系统的重要平台之一。
% ，最初于 1987 年由理查德·斯托曼（Richard Stallman）为 GNU 操作系统项目编写。GCC 支持 C、C++、Objective-C、Fortran、Ada、Go、D 语言等多种编程语言，并可生成多种目标架构（包括 x86、ARM、RISC-V、PowerPC 等）的机器代码。

\subsubsection{Instrumentation-Based Profile-Guided Optimization}
% \subsubsection{基于插桩的反馈优化}

GCC's PGO uses compile-time instrumentation and a two-phase build process. In the first phase (profile generation), the program is compiled with \texttt{-fprofile-generate} (or \texttt{-fprofile-arcs}), instrumenting branches, loops, and function calls to record their execution counts. Running the instrumented binary under training workloads produces profile data files (\texttt{.gcda} and \texttt{.gcno}) containing basic-block and branch counts. In the second phase (profile use), the program is recompiled with \texttt{-fprofile-use}, and GCC reads the collected profile data to guide optimizations.
% GCC 12.2的传统FDO采用编译时插桩和两阶段构建模式。第一阶段（程序描述信息生成）使用-fprofile-generate（或-fprofile-arcs）编译程序，通过插桩记录分支、循环和函数调用等指令的的执行次数。当插桩后的二进制文件在训练负载下运行时，会生成包含基本块和分支计数的程序描述信息文件（.gcda和.gcno文件）。第二阶段（程序描述信息使用）使用 -fprofile-use 重新编译程序，GCC 读取收集的描述性信息中的数据并应用反馈信息指导优化。

Internally, GCC annotates its intermediate representations (GIMPLE/RTL) with execution frequencies. These branch probabilities inform later passes, for example, the instruction scheduler and code-layout stages reorder basic blocks along the most likely paths to improve ICache utilization. Cold code (blocks or functions never executed in the profile) is laid out compactly or placed into separate “cold” sections. In fact, GCC by default can split functions into hot and cold parts with options like \texttt{-fprofile-reorder-functions} when using FDO.
% GCC内部利用程序描述信为中间表示（GIMPLE/RTL）标注执行频率：编译器将对中间表示附加分支概率和基本块执行计数。例如，GCC 会为每个分支指令设置 REG\_BR\_PROB （分支概率）属性而非依赖静态启发式分析算法的结果。这些执行概率将指导后续优化——如指令调度器和代码布局过程会按可能路径顺序排列基本块，提升指令缓存利用率。冷代码（描述信息中未执行的块或函数）会被优化为紧凑布局甚至放入独立的"冷"区段。实际上，GCC 默认在使用FDO时甚至可通过选项如-fprofile-reorder-functions将函数的热/冷部分拆分到不同区段。

Because instrumentation yields highly precise profile data, GCC also performs value-based optimizations—such as tracking indirect-call targets to promote virtual-call devirtualization. With \texttt{-fprofile-use} enabled, GCC aggressively applies full loop unrolling, loop peeling, deep inlining, and other high-level optimizations. Its inlining heuristics prioritize hot call sites while avoiding cold ones; hot loops are more likely to be unrolled or vectorized, whereas cold paths may be left unmodified.
% 由于插桩获取的程序描述信息精度极高（可细化到每个分支），GCC 12.2还能进行值分析——例如追踪间接调用目标，从而实现间接调用提升等值依赖优化。启用-fprofile-use后，GCC会激进启用全循环展开、循环剥离、深度内联等高等级优化。内联启发式算法会优先处理高频调用点，而冷调用则被规避。热循环更易被展开或向量化，冷路径则可能完全不作展开。

LLVM (with Clang as the front end) implements profile-guided optimization at the IR level using a similar two-step workflow. Compiling with \texttt{-fprofile-generate} inserts counters into the LLVM-IR to record basic-block and edge counts. After a training run, the resulting \texttt{.profraw} files are merged into a \texttt{.profdata} profile using the \texttt{llvm-profdata} tool. The optimization phase, invoked with \texttt{-fprofile-use}, loads the profile data; the LLVM back end then attaches execution counts as LLVM-IR metadata.
% LLVM 15（以 Clang 为前端）通过 IR 层插桩以及与 GCC 相同的二次编译形式实现反馈优化。使用 -fprofile-generate 编译时，编译器在 LLVM-IR 中插入计数器记录基本块和边的执行次数。训练运行后生成的 .profraw 文件经 llvm-profdata 工具合并为 .profdata 程序描述信息。优化阶段使用 -fprofile-use 加载程序描述信息，LLVM 后端将执行计数附加为 LLVM-IR 元数据（如分支权重）。
LLVM uses its own \texttt{.profdata} format, which is not compatible with the one in GCC.  Based on the profile data, LLVM also adjusts its optimization strategies: the inliner becomes more aggressive on hot calls, loop optimizations choose unrolling strategies according to hotness, and cold code may be isolated. Basic-block layout uses branch probabilities to guide cache-friendly ordering.
% 基于程序描述信息，LLVM 也会对优化策略进行调整，如：内联器对热点调用更激进，循环优化根据热度决定展开策略，冷点代码可能被外联。基本块布局按分支概率优化缓存顺序。与GCC不同，LLVM使用专属 .profdata 格式，且不兼容GCOV。
% 在 GCC 中基于插桩的反馈优化由编译时插桩以及二次编译两部分实现。在第一阶段，用户需要使用 $-fprofile-generate$ （或是 $-fprofile-arcs$) 选项编译程序。在这一阶段，编译器将自动插入统计分支、循环、函数调用的统计可执行片段。当一次编译程序被执行时，将生成程序描述性信息（通常为 $.gcda$ 以及 $.gcno$ 文件），包含各个基本块以及分支语句的执行情况。在二次编译时，用户需要使用 $-fprofile-use$ 选项第二次编译程序，这将使编译器读取并收集所需要的程序剖析信息，并应用于反馈优化所对应的优化过程中。在编译器内部，GCC 将程序描述信息用来标注中间语言（GIMPLE/RTL）的执行频率。比如 GCC 将对每个分支的 $REG_BR_PROB$ 属性进行真实执行信息标注，而非使用静态推断信息。所标注的可能性信息将被用来指导后续优化。如在内敛决策中，优化器将对热点调用进行更为激进的内联处理。在循环优化中，根据循环执行是否频繁而进行展开或是剥离。在向量化中，使用动态成本模型（$-fvect-cost-model=dynamic$）判断是否需要矢量化。在对于代码布局的优化中，通过在各个优化过程中（$-fprofile-reorder-functions$ 等）将热代码块集中分布，而将冷代码段分离到冷段之中。对于间接调用，通过值采样，将频繁被执行的间接调用直接内联化处理。

\subsubsection{Sampling-Based Profile-Guided Optimization}
% \subsubsection{基于采样的反馈优化}

Sampling-based feedback optimization replaces explicit instrumentation with hardware-event sampling (typically via the PMU). The typical workflow is: after a normal compile (with debug info), run the target under a performance profiler (e.g., \texttt{perf} with branch sampling enabled) to collect samples, then convert the sample data into a profile file.
%For example, on Intel hardware one might sample \texttt{br\_inst\_retired:near\_taken} to gather branch samples.
% 基于采样的反馈优化通过采样硬件事件（通常来自硬件计数器 PMU）替代显式插桩记录。典型流程为：常规编译程序（带调试信息）之后通过性能分析工具（如支持分支采样的perf）运行目标程序，最后将采样数据转换为程序描述文件。例如在Intel硬件上通常通过采样 br\_inst\_retired:near\_taken 采集分支样本。

In GCC, the raw data (\texttt{perf.data}) is converted into a GCC-readable \texttt{.afdo} file using the \texttt{create\_gcov} tool from the Google AutoFDO project. The final build uses \texttt{-fauto-profile}, which enables the same family of optimizations as \texttt{-fprofile-use} but driven by the sampled data.
% 在 GCC 中，数据（perf.data）随后通过 Google AutoFDO 项目提供的 create\_gcov 工具转换为 GCC 可读的 gcov格式 .afdo 文件。最终编译时使用 -fauto-profile=profile.afdo 启用与 -fprofile-use 相同的优化族（循环剥离、内联等），但使用的数据基于采样数据驱动。

GCC’s AutoFDO implementation comprises three stages: first, the compiler reads the profile and builds a mapping from function identifiers to profile records, creating a “function instance” forest that represents calling contexts; next, it performs an early optimization pass—before standard inlining—where it force-inlines hot call sites (ignoring code growth) and promotes frequently sampled indirect calls to direct calls; finally, it annotates the program’s CFG with sample counts, distributing counts to edges and nodes and estimating block frequencies and branch probabilities. This achieves performance comparable to traditional PGO while avoiding instrumentation overhead.
% 在 GCC 内部 AutoFDO 的实现包含三个阶段: 首先，编译器对描述信息进行读取，并构建以函数为单位的标识符到描述信息的映射，并创建表示函数上下文的"函数实例"森林；之后进行简单的早期优化，即在标准内联过程前，根据采样获得的程序描述信息强制内联高频调用点（无视代码膨胀），并提升高频间接调用为直接调用；最后，对程序控制流图 CFG 进行标注，将采样计数分配到控制流图中的边与节点，并估算基本块频率和分支概率。最终实现与传统PGO相近的优化效果，同时避免插桩构建的开销。%据早期报告可达插桩FDO 50-110%的性能提升（arxiv.org），同时避免插桩构建的开销。

% Internally, GCC’s AutoFDO implementation comprises three stages:
% \begin{enumerate}
%   \item Read the profile and build a mapping from function identifiers to profile data, creating a “function-instance” forest to represent calling contexts.
%   \item Perform early “forced” optimizations before standard inlining: aggressively inline hot call sites (ignoring code-size growth) and devirtualize frequent indirect calls.
%   \item Annotate the CFG with sampled counts, distributing samples to edges and nodes, and estimate basic-block frequencies and branch probabilities.
% \end{enumerate}
% This achieves optimization quality close to traditional PGO while avoiding instrumentation overhead.


LLVM 15 follows a similar pattern: compile with debug info, then sample with \texttt{perf} and convert the data via \texttt{llvm-profgen} into a \texttt{.prof} file. The second compile uses \texttt{-fprofile-sample-use}. A key difference is that LLVM’s \texttt{SampleProfileLoader} performs profile-guided inlining at IR-metadata-attachment time (analogous to GCC’s early inlining), uses the Profi algorithm \cite{10.1145/3498714} to infer missing edge counts, and supports context-sensitive sampling PGO by distinguishing function contexts via call-stack information.
% LLVM 15 同样采用首先进行带调试信息编译（-fdebug-info-for-profiling），之后通过 perf 采样并使用 llvm-profgen 工具转换采样数据为 .prof 文件，最后使用 -fprofile-sample-use 选项进行二次编译。与 GCC 中基于采样的反馈优化的关键差异在于：在 LLVM 中读取程序描述信息时 （SampleProfileLoader） 在标注 IR 频率的同时执行程序描述信息引导的内联优化（类似GCC早期内联阶段），并采用 Profi 算法推断缺失边计数；同时支持上下文敏感采样 PGO（CSSPGO），并通过调用栈信息区分函数上下文。


% 在编译阶段，GCC 12.2 和 LLVM 15 都将性能分析数据直接注入前端和优化流水线。GCC 的传统插桩式 PGO 通过 -fprofile-generate 和 -fprofile-use 驱动，支持基于精确执行次数的细粒度优化，例如分支概率标注、循环展开和值特化。其 AutoFDO 工作流（通过 -fauto-profile 激活）遵循相同的优化逻辑，但使用 Linux perf 等外部工具生成的采样数据。LLVM 的行为与之对应：插桩式 PGO 使用 -fprofile-instr-generate 和 -fprofile-instr-use 指导 IR 层基本块重排和内联优化，而 AutoFDO（-fprofile-sample-use）则将采样事件映射回 IR 进行类似的代码布局和内联决策。



As illustrated in Figure~\ref{fig:pgo_phase_comparison}, both GCC 12.2 and LLVM 15 inject profiling data into their front-ends and optimization pipelines during compile time. GCC enables fine-grained optimizations based on precise counts, such as branch probability annotation, loop unrolling, and value specialization. LLVM corresponds by using PGO to guide IR-level block reordering and inlining. When Link-Time Optimization (LTO) is enabled, both compilers propagate profile data across translation units: GCC’s LTO performs whole-program inlining and layout optimizations to ensure hotspots are optimized across modules, while LLVM’s IR-level LTO channel consumes the merged \texttt{.profdata} to drive cross-procedural hot/cold code placement. By default, neither compiler includes post-link binary rewriting, but both ecosystems support external tools—such as Meta’s BOLT or LLVM’s Propeller—that operate on the final executable, using the compiler’s profile data (instrumentation or sampling) to optimize code layout, reduce ICache misses, and improve branch prediction. Integrated into the toolchain, these tools add an optional post-link optimization stage complementary to compile-time and link-time PGO.
% 如图 \ref{fig:pgo_phase_comparison} 所示，在编译阶段，GCC 12.2 和 LLVM 15 都将性能分析数据直接注入前端和优化流水线。GCC 支持基于精确执行次数的细粒度优化，例如分支概率标注、循环展开和值特化。LLVM 的行为与之对应：插桩式 PGO 指导 IR 层基本块重排和内联优化。在链接阶段启用链接时优化（LTO）时，两个编译器都会跨翻译单元传播性能分析信息。GCC 的 LTO 会合驱动全程序内联和代码布局优化，确保跨模块的热点函数被整体优化。LLVM 的链接时分析数据使用方式类似：合并后的 .profdata 会输入到 IR 层 LTO 通道，实施符合运行时观测的热/冷代码区分的跨过程优化。默认情况下，两个编译器均不内置链接后的二进制重写功能。但两者生态都支持外部二进制优化工具，如 Meta 的 BOLT 或 LLVM 的 Propeller。这些工具作用于最终可执行文件，但只能使用 LLVM 支持的分析数据（插桩或采样）优化代码布局、减少指令缓存未命中、提升分支预测精度。当集成到工具链时，它们提供可选的链接后优化阶段，与编译时和链接时的 PGO 形成互补。

Overall, core PGO and AutoFDO mechanisms act during compile and LTO phases, while advanced binary layout optimizations are performed post-link by dedicated tools. This multi-stage, collaborative strategy ensures that profiling feedback informs high-level code transformations and low-level binary organization, maximizing runtime performance in large software systems.
% 总体而言，核心 PGO 和 AutoFDO 机制主要作用于编译期和 LTO 阶段，而高级二进制布局优化则通过专用工具在链接后实施。这种多阶段协同策略使性能反馈数据既能塑造高级代码转换，又能优化底层二进制组织，最终在大型软件系统中实现最大化的运行时性能提升。


\input{contents/figs/gcc-vs-llvm.tex}
